Unleashing the Power of Compiler Intermediate Representation to Enhance Neural Program Embeddings

Neural program embeddings have demonstrated considerable promise in a range of program analysis tasks, including clone identification, program repair, code completion, and program synthesis. However, most existing methods generate neural program embeddings directly from the program source codes, by learning from features such as tokens, abstract syntax trees, and control flow graphs. This paper takes a fresh look at how to improve program embeddings by leveraging compiler intermediate representation (IR). We first demonstrate simple yet highly effective methods for enhancing embedding quality by training embedding models alongside source code and LLVM IR generated by default optimization levels (e.g., -O2). We then introduce IRGen, a framework based on genetic algorithms (GA), to identify (near-)optimal sequences of optimization flags that can significantly improve embedding quality.

==> alluppermath-notations.tex <==
%{math-notations}

% natural numbers
\newcommand{\NATURALS}{{\rm Nat}}

% functions names inside of math environment
\newcommand{\fun}[1]{\hbox{\it #1\/}}

% brackets that surround syntax (as in denotational semantics)
\newcommand{\synbracket}[1]{[\![{#1}]\!]}

% logic
\newcommand{\IFF}{\Leftrightarrow}
\newcommand{\DEF}{\stackrel{{\rm def}}{=}}
\newcommand{\DEFEQUIV}{\stackrel{{\rm def}}{\equiv}}
\newcommand{\DEFIFF}{\stackrel{{\rm def}}{\IFF}}

% lambda calculus
\newcommand{\LAMBDA}[1]{\lambda{#1}\:.\:}
\newcommand{\FREEVARS}[1]{{\it FV\/}\synbracket{#1}}	% free variables
\newcommand{\FREEIDS}[1]{{\it FreeIds\/}(#1)}	% free identifiers
\newcommand{\SYNTAXWITHFOR}[3]{[#2/#3]#1}	% subst #2 for #3 in #1
\newcommand{\WITHFOR}[3]{#1[#2/#3]}		% subst #2 for #3 in #1
\newcommand{\BETAREDUCESTO}{\stackrel{\beta}{\Rightarrow}}
\newcommand{\ETAREDUCESTO}{\stackrel{\eta}{\Rightarrow}}
\newcommand{\DELTAREDUCESTO}{\stackrel{\delta}{\Rightarrow}}
\newcommand{\BETAEQUALS}{\stackrel{\beta}{=}}
\newcommand{\ETAREQUALS}{\stackrel{\eta}{=}}
\newcommand{\DELTAEQUALS}{\stackrel{\delta}{=}}

% higher order lambda calculus
\newcommand{\POLY}[1]{\Lambda{#1}\:.\:}
\newcommand{\ALLTYPE}[1]{\forall{#1}\:.\:}
\newcommand{\EXISTSTYPE}[1]{\exists{#1}\:.\:}
\newcommand{\DEPFUNTYPE}[1]{\Pi{#1}\:.\:}
\newcommand{\DEPSUMTYPE}[1]{\Sigma{#1}\:.\:}

% recursion theory
\newcommand{\ZEROORMORE}[1]{{#1}^{\rm *}}
\newcommand{\ONEORMORE}[1]{{#1}^{+}}

% category theory
\newcommand{\DOM}[1]{{\it Domain\/}(#1)}
\newcommand{\POWERSET}[1]{{\it PowerSet\/}(#1)}

% topology
\newcommand{\CLOSURE}[1]{\overline{#1}}
\newcommand{\LUB}{{\rm lub}}			% least upper bound

% set theory
\def\elem{\hbox{\raise.13ex\hbox{$\scriptstyle\in$}}}
\newcommand{\GRAPH}{{\it graph}}

% relations
\newcommand{\RELATIONTYPE}[1]{2^{(#1)}}


==> calculation.tex <==
% $Id: calculation.tex 2 2008-12-23 22:46:05Z gary.leavens $
%
% Calculational proofs, a la Dijkstra, Gries, Back and von Wright, etc.
% See: David Gries, "Teaching Calculation and Discrimination:
%      A More Effective Curriculum", CACM 34(3):44-55, Mar. 1991.
% and
%      Ralph-Johan Back and Joakim von Wright,
%      "Refinement Calculus: A Systematic Introduction",
%      Springer-Verlag, 1998.
%
% AUTHOR: Gary T. Leavens

% EXAMPLES
%
% A simple example of the use of these macros is as follows.
%
% \begin{calculation}
% \FORMULA{\vec{RD}}
% \EQREASON{definition of $\vec{RD}$}
% \FORMULA{(RD_1, \ldots, RD_j, \ldots, RD_{12})}
% \REASON{\sqsubseteq}{$F_j$ is monotonic}
% \FORMULA{(RD_1, \ldots, F_j(\vec{RD}), \ldots, RD_{12})}
% \EQREASON{definition of $\vec{RD'}$}
% \LASTFORMULA{\vec{RD'}}
% \end{calculation}
%
% The following is a slightly more advanced example.
%
% \begin{calculation}
% \FORMULA{F(\vec{RD'}) \sqsubseteq \FOCUS{F^n(\vec{\emptyset})}}
% \EQREASON{assumption $F^n(\vec{\emptyset}) = F^{n+1}(\vec{\emptyset})$}
% \FORMULA{F(\vec{RD'}) \sqsubseteq \FOCUS{F^{n+1}(\vec{\emptyset})}}
% \EQREASON{definition of iteration of a function}
% \FORMULA{F(\vec{RD'}) \sqsubseteq F(F^n(\vec{\emptyset}))}
% \REASON{\impliedby}{monotonicity of $F$}
% \FORMULA{\vec{RD'} \sqsubseteq F^n(\vec{\emptyset})}
% \REASON{\impliedby}{transitivity}
% \FORMULA{\vec{RD'} \sqsubseteq F(\vec{RD})
%         \wedge F(\vec{RD}) \sqsubseteq F^n(\vec{\emptyset})}
% \EQREASON{assumption $F(\vec{RD}) \sqsubseteq F^n(\vec{\emptyset})$}
% \FORMULA{\vec{RD'} \sqsubseteq F(\vec{RD})}
% \REASON{\impliedby}{Lemma~7}
% \QEDFORMULA{\vec{RD} \sqsubseteq F(\vec{RD})}
% \end{calculation}
%
% An much more sophisticated example, with subdeductions a la Back and
% von Wright is the following.
%
% \begin{calculation}
% \FORMULA{\alpha(\{tr: (z, \ell') \mid tr \in \gamma(RD_k)\}) }
% \EQREASON{definition of $\alpha$}
% \FORMULA{\{(x, SRD(tr')(x))
%              \mid x \in \textrm{dom}(tr')
%                   \wedge tr' \in \{tr: (z, \ell') \mid tr \in \gamma(RD_k)\} \} }
% \EQREASON{set theory
%          ($tr'$ ranges over $tr: (z, \ell')$ for $tr \in \gamma(RD_k)$)}
% \FORMULA{\{(x, SRD(tr: (z, \ell'))(x))
%              \mid x \in \textrm{dom}(tr: (z, \ell')),
%                    \FOCUS{tr \in \gamma(RD_k)} \} }
% \EQREASON{definition of $\gamma$}
% \FORMULA{\{(x, SRD(tr: (z, \ell'))(x))
%              \mid x \in \textrm{dom}(tr: (z, \ell')),
%                (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \}}
% \EQREASON{set theory}
% \FORMULA{
%     \begin{array}{rl}
%         \{(x, SRD(tr: (z, \ell'))(x)) &
%              \mid x \neq z, x \in \textrm{dom}(tr: (z, \ell')), \\
%              & ~ (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \} \\
%         \cup \:
%         \{(x, SRD(tr: (z, \ell'))(x)) &
%              \mid x = z, x \in \textrm{dom}(tr: (z, \ell')), \\
%              & ~ (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \}
%     \end{array}
%         }
% \EQREASON{focusing on the second set}
% \SUBDEDUCTION{
%      \begin{array}{rl}
%         \{(x, SRD(tr: (z, \ell'))(x)) &
%              \mid x = z, x \in \textrm{dom}(tr: (z, \ell')), \\
%              & ~ (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \}
%      \end{array}
%        }
%   \EQREASON{set theory}
%   \FORMULA{\{(z, \FOCUS{SRD(tr: (z, \ell'))(z)}) 
%              \mid z \in \textrm{dom}(tr: (z, \ell')),
%                (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \} }
%   \EQREASON{definition of $SRD$}
%   \FORMULA{\{(z, \ell') 
%              \mid \FOCUS{z \in \textrm{dom}(tr: (z, \ell'))},
%                (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k)
%              \} }
%   \EQREASON{definition of $\textrm{dom}$}
%   \FORMULA{\{(z, \ell') 
%              \mid (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \} }
%   \EQREASON{definition of $\gamma$}
%   \FORMULA{\{(z, \ell') \mid tr \in \gamma(RD_k) \} }
%   \EQREASON{$tr$ can be constructed by writing the pairs of
%              $\gamma(RD_k)$ in some order}
%   \FORMULA{\{(z, \ell') \} }
% \CONCLUDE{
%    \begin{array}{l}
%     \begin{array}{rl}
%         \{(x, SRD(tr: (z, \ell'))(x)) &
%              \mid x \neq z, x \in \textrm{dom}(tr: (z, \ell')), \\
%              & ~ (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \}
%     \end{array} \\
%     \cup \: \{(z, \ell')\}
%    \end{array}
%     }
% \EQREASON{focusing on the first set}
% \SUBDEDUCTION{
%     \begin{array}{rl}
%         \{(x, SRD(tr: (z, \ell'))(x)) &
%              \mid x \neq z, x \in \textrm{dom}(tr: (z, \ell')), \\
%              & ~ (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \}
%      \end{array}
%        }
%   \EQREASON{definition of $SRD$}
%   \FORMULA{\{(x, SRD(tr)(x))
%              \mid x \neq z, x \in \textrm{dom}(tr), 
%               (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \}}
%   \EQREASON{set theory and the range of $SRD$}
%   \FORMULA{\begin{array}{l}
%              \{(x, SRD(tr)(x))
%                       \mid x \in \textrm{dom}(tr), 
%               (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \} \\
%            \setminus \: \{(z, \ell) \mid \ell \in \Lab\}
%            \end{array}
%           }
%   \EQREASON{Lemma \ref{lemma:simplifyToRD}}
%   \FORMULA{RD_k \setminus \{(z, \ell) \mid \ell \in \Lab\}}
% \LASTCONCLUDE{(RD_k \setminus \{(z, \ell) \mid \ell \in \Lab\})
%            \cup \{(z, \ell')\}}
% \end{calculation}


%%%%%%% The macros themselves follow %%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% You may want to define the following with \renewcommand...

% Brackets around normal and fixed width reasons
\newcommand{\LEFTREASONBRACKET}{\langle}
\newcommand{\RIGHTREASONBRACKET}{\rangle}
% Brackets for long reasons
\newcommand{\LONGLEFTREASONBRACKET}{\left\LEFTREASONBRACKET}
\newcommand{\LONGRIGHTREASONBRACKET}{\right\RIGHTREASONBRACKET}
% width of long and fixed width reasons
\newcommand{\LONGREASONWIDTH}{5.4in}
\newcommand{\FIXEDWIDTHREASONWIDTH}{\LONGREASONWIDTH}
% The phrase that starts each reason
\newcommand{\BYPHRASE}{by~}
% Provability symbol
\newcommand{\PROVABILITYSYMBOL}{\vdash}
% Has type symbol
\newcommand{\CALCULATIONHASTYPE}{:}
% Subdeduction symbols a la Back and von Wright
\newcommand{\SUBDEDUCTIONMARKER}{\bullet}
\newcommand{\CONCLUDEMARKER}{\cdot}

% The macros below assume that you have defined \QED,
% e.g., as \newcommand{\QED}{q.e.d.}


%%% The rest shouldn't usually need to be redefined

% The main environment
\newenvironment{calculation}{
\samepage
\begin{tabbing}
n \= n \= n \= n \= mm \= n \= mm \= n \= mm \= n \= mm \= n \= mm \= \kill
}{
\end{tabbing}
}

% Use for the last formula (to avoid extra vertical space)
\newcommand{\LASTFORMULA}[1]{\> \ensuremath{#1}}
% Use for the last formula in a proof that concluses the proof
\newcommand{\QEDATEND}{~~\QED}
\newcommand{\QEDFORMULA}[1]{\LASTFORMULA{#1\QEDATEND}}

% All other formulas in a calculation
\newcommand{\FORMULA}[1]{\LASTFORMULA{#1} \\}

% Generic reason, with connective and the justification
\newcommand{\REASON}[2]{%
    \ensuremath{#1}\> \>
       \mbox{\ensuremath{\LEFTREASONBRACKET}{\BYPHRASE}#2\ensuremath{\RIGHTREASONBRACKET}} \\}

% Reasons with longer justifications, with the right bracket at the end
\newcommand{\FIXEDWIDTHREASON}[2]{%
     \ensuremath{#1}\> \>
       \ensuremath{\LEFTREASONBRACKET}{\BYPHRASE}%
       \parbox[t]{\FIXEDWIDTHREASONWIDTH}{#2\ensuremath{\RIGHTREASONBRACKET}}
       \\
     }

% Reasons with longer justifications, with big brackets around the reason
\newcommand{\LONGREASON}[2]{%
    \ensuremath{#1}\> \>
      \ensuremath{\LONGLEFTREASONBRACKET
                  \parbox[c]{\LONGREASONWIDTH}{{\BYPHRASE}#2}
                  \LONGRIGHTREASONBRACKET
                 }
      \\
    }

% Specialization of reasons to equality
\newcommand{\EQREASON}[1]{\REASON{=}{#1}}
\newcommand{\EQLONGREASON}[1]{\LONGREASON{=}{#1}}
\newcommand{\EQFIXEDWIDTHREASON}[1]{\FIXEDWIDTHREASON{=}{#1}}

% Use \FOCUS{E} to say that subformula E will be changed in the following step
\newcommand{\FOCUS}[1]{\mbox{``}#1\mbox{''}}


%% The following are for Back and von Wright style calculations.
%% First time users may want to ignore these.

% Use for assumptions in a type-deduction style proof
\newcommand{\GIVEN}[1]{\FORMULA{#1}}
% Use \PROVETHAT to start the body of a type-deduction style proof.
\newcommand{\PROOFLINE}[2]{\ensuremath{#1} \> \ensuremath{#2} \\}
\newcommand{\PROVETHAT}[1]{\PROOFLINE{\PROVABILITYSYMBOL}{#1}}
%% Subdeductions
% Use to start a subdeduction
\newcommand{\SUBDEDUCTION}[1]{\+\+\kill\PROOFLINE{\SUBDEDUCTIONMARKER}{#1}}
% Use to separate one subdeduction from another
\newcommand{\ANDALSO}{\-\-\kill}
% Use to start the next subdeduction after \ANDALSO
\newcommand{\NEXTDEDUCTION}[1]{\PROOFLINE{\SUBDEDUCTIONMARKER}{#1}}
% Use to conclude a subdeduction 
\newcommand{\CONCLUDE}[1]{\-\-\kill\PROOFLINE{\CONCLUDEMARKER}{#1}}
% Use when the last formula is also a conclusion
\newcommand{\LASTCONCLUDE}[1]{\-\-\kill\ensuremath{\CONCLUDEMARKER} \> \ensuremath{#1}}
% Use in a type-deduction proof instead of \REASON, to give the rule name
\newcommand{\TYPINGRULE}[1]{\ensuremath{\CALCULATIONHASTYPE} \> ~~~ #1 \\}

% end of calculation.tex


==> denotational-semantics.tex <==
% requires math-notations

% Typography as in Schmidt's book: Denotational Semantics.
% Many of the following defs must be used in a math environment; all can be.

% natural numbers: \NATURALS
\renewcommand{\NATURALS}{{\it Nat}}
\newcommand{\ZERO}{{\it zero}}
\newcommand{\ONE}{{\it one}}
\newcommand{\TWO}{{\it two}}
\newcommand{\THREE}{{\it three}}
\newcommand{\FOUR}{{\it four}}
\newcommand{\PLUS}{{\it plus}}
\newcommand{\MINUS}{{\it minus}}
\newcommand{\TIMES}{{\it times}}
\newcommand{\EQUALNATURALS}{{\it equals}}

% integers: \INTEGER
\newcommand{\INTEGER}{{\it Int}}
\newcommand{\ADDR}{{\it Addr}}

% Booleans: \BOOLEAN
\newcommand{\BOOLEAN}{{\it Boolean}}
\newcommand{\TRUE}{{\it true}}
\newcommand{\FALSE}{{\it false}}
\newcommand{\NOT}{{\it not}}
\newcommand{\OR}{{\it or}}
\newcommand{\AND}{{\it and}}
\newcommand{\IFEXP}[3]{#1 \rightarrow #2 [\!] #3 }
\newcommand{\IFHEAD}[1]{#1 \rightarrow}
\newcommand{\IFELSE}{[\!]~}

% truth values
\newcommand{\TR}{{\it Tr}}
\newcommand{\TT}{{\it tt}}
\newcommand{\FF}{{\it ff}}

% Strings: \STRING
\newcommand{\STRING}{{\it String}}
\newcommand{\EMPTYSTRING}{{\it empty}}
\newcommand{\ERRORSTRING}{{\it error}}
\newcommand{\CONCATSTRINGS}{{\it concat}}
\newcommand{\LENGTHOFSTRING}{{\it length}}
\newcommand{\SUBSTRING}{{\it substr}}		% 3 arguments

% other primitive domains
\newcommand{\UNIT}{{\it Unit}}
\newcommand{\ERROR}{{\it Error}}

% other standard semantics domain names
\newcommand{\ANSWERS}{{\it Answer}}
\newcommand{\CMDCONT}{{\it Cmdcont}}
\newcommand{\DENOTABLE}{\mbox{\it Denotable-value}}
\newcommand{\ENVIRONMENT}{{\it Environment}}
\newcommand{\EXPRESSIBLE}{\mbox{\it Expressible-value}}
\newcommand{\EXPCONT}{{\it Expcont}}
\newcommand{\LOCATION}{{\it Location}}
\newcommand{\PROCEDURE}{{\it Procedure}}
\newcommand{\REFERENCE}{{\it Reference}}
\newcommand{\RESULT}{{\it Result}}
\newcommand{\STORE}{{\it Store}}
\newcommand{\STORABLE}{\mbox{\it Storable-value}}
\newcommand{\UNBOUND}{{\it Unbound}}
\newcommand{\VALUE}{{\it Value}}

% disjoint union: $A + B$
\newcommand{\INJECTION}[1]{{\rm in}\!{#1}}
\newcommand{\ISTEST}[1]{{\rm is}\!{#1}}
\newcommand{\CASEHEAD}[1]{\mbox{{\bf cases} ${#1}$ {\bf of} }}
\newcommand{\CASE}[2]{{#1} \:\rightarrow\: {#2}}
\newcommand{\CASESEP}{[\!]}
\newcommand{\CASEELSE}{\mbox{{\bf else} }}
\newcommand{\CASEEND}{{\bf end}}

% product space: $A \times B$
\newcommand{\PAIR}[2]{({#1},{#2})}
\newcommand{\FST}{{\it fst}}
\newcommand{\SND}{{\it snd}}
\newcommand{\ATINDEX}[2]{#1 \downarrow #2}
% Note $\ZEROORMORE{A} = Unit + A + (A \times A) + (A \times A \times A) + ...$
% Lists are $Unit + A + (A \times A) + (A \times (A \times A)) + ...$

% list space: $\LIST{A}$
\newcommand{\LIST}[1]{{\it List}(#1)}
\newcommand{\LNIL}{{\it nil}}
\newcommand{\LCONS}{{\it cons}}
\newcommand{\LHEAD}{{\it hd}}
\newcommand{\LTAIL}{{\it tl}}
\newcommand{\LNULL}{{\it null}}

% function space: $A \rightarrow B$
\newcommand{\UPDATEFUN}[3]{[{#1} \mapsto {#2}]{#3}}

% finite functions
\newcommand{\FINITEARROW}{\stackrel{{\rm fin}}{\rightarrow}}

% lifted domain: $\LIFT{A}$
\newcommand{\LIFT}[1]{{#1}_{\bot}}
\newcommand{\STRICTLAMBDA}[1]{\underline{\lambda}{#1}\:.\:}
\newcommand{\LETHEAD}[2]{\mbox{{\bf let} }{#1} = {#2}\mbox{ {\bf in} }}
\newcommand{\MAP}[2]{\mbox{{\bf map} }{#1} => {#2\{#1\}}}

% fixpoints
\newcommand{\FIX}{{\it fix}}

% common valuation functions
\newcommand{\MEANING}[2]{{\cal #1}\synbracket{#2}}
\newcommand{\DENEXPRESSION}[1]{\MEANING{E}{#1}}
\newcommand{\DENCOMMAND}[1]{\MEANING{C}{#1}}
\newcommand{\DENLITERAL}[1]{\MEANING{L}{#1}}
\newcommand{\DENPROGRAM}[1]{\MEANING{P}{#1}}

% an environment for typesetting
\newenvironment{DENOTATIONAL}{%
\samepage
\begin{tabbing}
mmm \= mmm \= mmm \= mmm \= mmm \= mmm \= mmm \= mmm \= \kill
}{
\end{tabbing}
}


==> fig/sample table and figure/5.1-evaluation.tex <==

\subsection{Experiments on Real-world Datasets}
\label{subsec:exp}
\subsubsection{Setup}

% \begin{table}[!htbp]
% \centering \caption{Dataset Statistics}
%    \label{tab:datasetstat}
%    \resizebox{0.8\linewidth}{!}{
%   \begin{tabular}{c|c|c|c|c|c}
%     \#Cells & 0-1k & 1k-10k & 10k-100k & 100k-1M & 1M+\\\hline
%     \#Datasets & 7 & 8 & 8 & 6 & 6\\
%     \Xhline{2\arrayrulewidth}
%     Domain & Sales & Finance & Environment & Healthcare &  Other\\\hline
%     \#Datasets & 9 & 5 & 3 & 3 & 15
%     \end{tabular}
%    }
% \end{table}

\noindent\textbf{Dataset.} We select 35 datasets from more than 10 domains 
(e.g., Sales, Environment and Healthcare) to evaluate the effectiveness 
and efficiency of \mi. These datasets are of different scales, ranging from 
one thousand cells to over one million cells. In particular, we pick four
large datasets to evaluate \mi's efficiency at the extreme. 

\noindent\textbf{Environment.} We conduct all experiments on Windows 10 with an Intel 
Core i7-8700 and 16 GB RAM. The \mi\ mining procedure is implemented by \Csharp, and 
we implement a plugin on Microsoft Excel to work with its query interface. 
We set the configuration as follows: \#worker threads = 8 and the maximal filter 
size in a subspace = 3. We set \texttt{COUNT(*)} as impact-measure for all datasets, 
for simplicity, and we note that the choice of impact-measure only has a negligible 
effect on evaluating efficiency. 

\subsubsection{Experiment Design}
\label{subsubsec:exp-design}
We evaluate \mi\ from two aspects, namely, the efficiency of the \mi\ mining 
procedure, and the optimality of our ranking algorithm.

% Specifically, to evaluate the effectiveness of \mii, we design 
% a metric called the \emph{knowledge density ratio} to measure the density of 
% knowledge presented by \mii\ vs. flat-list representation. The metric is defined 
% as follows.

% \begin{definition} (Knowledge density ratio)
%     \begin{equation}
%         R=\frac{n}{\abs{\texttt{CommSet}}+\abs{\texttt{exceptions}}}
%     \end{equation}
% \end{definition}

% \noindent where $\abs{\texttt{CommSet}}$ and $\abs{\texttt{exceptions}}$ are the number of 
% commonnesses and exceptions, respectively. The flat-list representation denotes that 
% data patterns in the given \mii\ are presented separately (similar to the middle 
% charts in \F~\ref{fig:usercase}). The knowledge represented by a \mii\ is deemed to be
% approximately equal to that representing the corresponding flat data patterns, i.e., flat-list 
% representation (this is supported by our user study in \S~\ref{subsec:userstudy}). 
% But the volumes occupied by these two representations are different. When conveying the 
% knowledge by flat-list representation, we need $n$ charts ($n$ is the number of data 
% patterns in the HDP of a \mii) to present it; when conveying the knowledge by a \mii, 
% we only need one chart for each commonness (since all the data patterns within a 
% commonness share the same characteristic); thus we need $\abs{\texttt{CommSet}}+
% \abs{\texttt{exceptions}}$ charts at most (without considering the categorization 
% of exceptions). We use $n$ and $\abs{\texttt{CommSet}}+\abs{\texttt{exceptions}}$ to 
% estimate the volumes to store the knowledge for flat-list representation and \mii, 
% respectively, and we have the definition of the \emph{knowledge density ratio}.


In terms of mining efficiency, we employ several optimizations to boost the search, 
query and evaluation functionalities. We conduct an ablation study by disabling 
one of the optimizations or replacing it with a baseline. Specifically, we compare 
the efficiency by using priority queues vs.~using FIFO queues, by enabling query cache 
vs.~disabling query cache, and enabling pattern cache vs.~disabling pattern cache. 
We define \mi\ precision to measure the effectiveness of each optimization. In addition, 
we also conduct end-to-end comparisons between \mi\ and \qi\ to evaluate \mi\ extra 
cost, since \mi\ conducts not only mining of basic data patterns (which \qi\ does),
but also mining of HDPs. We use total number of emitted queries as metric which 
reflects major performance cost.

\begin{definition} (\mi\ Precision)
    Let $\mathcal{M}$ and $\mathcal{M}_0$ denote two sets of \mis,
    where $\mathcal{M}_0$ is the golden set and $\mathcal{M}$ is 
    the comparative set. The \mi\ precision $\beta$ is 
    \begin{equation}
        \beta=\frac{\abs{\mathcal{M}_0\cap\mathcal{M}}}{\abs{\mathcal{M}_0}}
    \end{equation}
\end{definition}

\noindent
In our golden setting, all optimizations are enabled and the time budget is 600 seconds. 
Then, we compare the golden set $\mathcal{M}_0$ with other results in different 
methods and compute \mi\ precisions. Each comparative method is repeated under 
different time budgets on four datasets. Higher precision denotes better performance. 
$\beta=1$ means that the mining procedure can achieve equivalent performance 
under this setting. As a part of our optimizations, in addition to \mi\ precision, 
we also report the statistics of the query cache and the pattern cache in the 35 
datasets to show how much communication and computational cost is saved.

To understand the optimality of our ranking algorithm, we first run a standalone 
baseline algorithm (neither second-order approximation or greedy algorithm is enabled) 
to find the globally optimal top-$k$ set of \E~\ref{eq:orig-ranking}. Then we use this 
set as the golden set, and evaluate the optimality of our ranking algorithm. We also 
compare our algorithm with a rank-by-score algorithm (sorting all the 
\mis\ by scores in descending order and picking the top-$k$ ones).

% \begin{figure}[!htbp] 
% \centering
% \includegraphics[width=0.55\columnwidth]{fig/compressionratehist.pdf}
% \caption{Knowledge Density Ratio Histogram}
% \label{fig:compression}
% \end{figure}

\subsubsection{Results}
\label{subsec:result}

% \F~\ref{fig:compression} reports the promising results of the knowledge density ratio of 
% \mis\ vs. flat-list representation on our 35 datasets, where the x-axis denotes the 
% knowledge density ratio, the left y-axis denotes the number of \mis\ with a certain knowledge
% density ratio and the right y-axis denotes the cumulative distribution function.
% The average knowledge density ratio in these datasets is 3.92, and all \mis\ 
% have a knowledge density ratio more than 2. Therefore, \mi\ representation 
% provides much convenience to convey structured knowledge compared with the
% flat-list representation.

\begin{figure}[!htbp]
\centering
\includegraphics[width=\columnwidth]{fig/exp/all.pdf}
\caption{Efficiency of \mi\ mining procedure (in terms of precision) under different datasets and settings}
\label{fig:coverage}
\end{figure}

% \begin{figure*}[!htbp]
% \centering
% \includegraphics[width=\textwidth]{fig/coverage.pdf}
% \caption{Efficiency of \mi\ (in terms of coverage) under different datasets and settings}
% \label{fig:coverage}
% \end{figure*}

\F~\ref{fig:coverage} reports the precision over different time budgets for 
the four different settings. 
The full functionality mining procedure achieves the best performance on all datasets 
among all time budgets. As we use the results of 600 seconds to be the golden set, 
we would like to note that the satisfactory results are generated in a much shorter time 
(e.g., the full functionality mining procedure achieves equivalent performance within 120s 
in the ``Sales Forecast'' dataset). However, when either of these optimizations is disabled, there is
notable performance degradation in most time budgets. We also find that, with the scale of 
the dataset growing,
the implications of optimizations become increasingly important to the overall performance.
In the ``Hotel Booking'' dataset (the largest dataset among the four, w/ 1M+ cells), the effectiveness of our optimizations 
is obvious. For 
a medium-sized dataset (w/ 100k-1M cells), e.g., the ``Tablet Sales'' dataset, when either of the caches is disabled, 
the mining procedure takes 12x longer (5s vs. 60s) to achieve the same performance, 
let alone the mining procedure without a priority queue. Also, the importance of the query cache 
is relatively smaller than the others for the medium-sized datasets; given enough time, the mining 
procedure can discover good \mis\ as well. However, as there are many duplicated
data pattern evaluations, the absence of pattern cache may greatly slow down the performance.

\begin{table}[!htbp]
\centering \caption{Cache Statistics}
   \label{tab:cache}
   \resizebox{0.6\linewidth}{!}{
  \begin{tabular}{c|c|c|c|c}
    \#Cells & \#$C_q$ & \textbf{$r_q$} & \#$C_p$ & \textbf{$r_p$}\\
    \Xhline{2\arrayrulewidth}
    0-1k      & 0.5  & 80.4\% & 179  & 26.0\%\\
    1k-10k    & 35.9 & 75.6\% & 7175 & 34.8\%\\
    10k-100k  & 38.5 & 65.8\% & 1497 & 37.9\%\\
    100k-1M   & 99.4 & 74.9\% & 5594 & 42.2\%\\
    1M+       & 294  & 70.6\% & 3584 & 50.1\%
    \end{tabular}
   }
\end{table}

\begin{figure}[!htbp]
\centering
\includegraphics[width=\columnwidth]{fig/query-count/query.pdf}
\caption{Query Count}
\label{fig:query}
\end{figure}

We use a total of 35 representative datasets to show the 
effectiveness of the query cache and pattern cache. We report the cache statistics in 
\T.~\ref{tab:cache}, where $\#C_q$ and $\#C_p$ denote the size of the query cache 
and pattern cache, respectively, and $r_q$ and $r_p$ denote the cache hit rate of the
query cache and pattern cache. Since the query cache employs a compound data structure 
(see \F~\ref{fig:queryunit}), $\#C_q$ is the memory size in \texttt{MB} (megabytes). 
As given in the table, a substantial number of data queries and 
pattern evaluations are eliminated by prefetching in the query cache and pattern cache.
On the ``Hotel Booking'' dataset, we find that more than 80\% of queries are prefetched
in the query cache, which explains the large performance degradation in 
\F~\ref{fig:coverage}(d). The results of the pattern cache hit rate also validate our statement
in \S~\ref{subsec:design-mining}, where data pattern evaluations are often duplicated 
(i.e., a basic data pattern may serve for different HDPs)..
For datasets with more than one million cells, more than half the data pattern evaluations are
saved. 

We further report the total emitted number of queries by \qi\ and \mi\ in \F~\ref{fig:query}. 
\mi\ conducts $17.1\%$ extra queries on average compared with \qi. On large datasets 
(\qi\ emits more than $10,000$ queries), the extra cost of \mi\ is only $7.9\%$ due to 
the better utilization of query and pattern cache. Overall, \mi\ has modest extra cost 
and is feasible to be integrated into production.


\begin{table}[!htbp]
\centering \caption{Optimality of \mi's Ranking}
   \label{tab:ranking}
    \resizebox{0.7\linewidth}{!}{
  \begin{tabular}{l|l|c|c|c}
    Dataset & Algorithm & Time & \texttt{TotalUse} & Precision\\
    \Xhline{3\arrayrulewidth}
    \multirow{3}*{Sales Forecast} & Baseline & >1min & 3.31& N/A \\
    \cline{2-5} & Our & 0.93 s & 3.27 & 0.90 \\
    \cline{2-5} & Rank-by-Score & 0.52 s & 2.48 & 0.40 \\ \Xhline{2\arrayrulewidth}
    \multirow{3}*{Tablet Sales} & Baseline & >1min &6.59 & N/A  \\
    \cline{2-5} & Our & 1.04 s & 6.59 & 1.0 \\
    \cline{2-5} & Rank-by-Score & 0.23 s & 4.23 & 0.30 \\ \Xhline{2\arrayrulewidth}
    \multirow{3}*{Credit Card} & Baseline & >1min& 8.52  & N/A  \\
    \cline{2-5} & Our & 1.90 s & 8.52 & 1.0 \\
    \cline{2-5} & Rank-by-Score & 0.36 s &4.82&0.30 \\ \Xhline{2\arrayrulewidth}
    \multirow{3}*{Hotel Booking} & Baseline & >1min &8.43& N/A  \\
    \cline{2-5} & Our & 2.37 s& 8.43 & 1.0 \\
    \cline{2-5} & Rank-by-Score & 0.39 s &3.78&0.30
    \end{tabular}}

\end{table}

% \T~\ref{tab:ranking} reports the results of the optimality of \mi's ranking algorithm
% compared with the baseline and rank-by-score algorithm. The results of our ranking 
% algorithm are in line with the baseline algorithm with full complexity in the above datasets.
% Owing to high-order redundancy being too small to have much of an effect on the 
% total usefulness, the second-order approximation sufficiently captures
% redundancy information, and we do not need to adopt the baseline algorithm, which 
% is much more costly. It is worth noting that the time usage of baseline is more than 
% one minute (even more than one hour in some datasets) which impedes its use
% in interactive EDA.
% However, if we do not take redundancy into account in the 
% ranking algorithm, i.e., the rank-by-score algorithm, the precision is much lower. In 
% terms of time usage, given the linear complexity of the greedy algorithm, our algorithm 
% also takes an acceptable time to give a plausible result.

\T~\ref{tab:ranking} reports the results of \mi\ ranking algorithm optimality
(second-order approximation) compared with baseline (accurate algorithm) and 
rank-by-score algorithm (first-order approximation). The results of our ranking 
algorithm are in line with baseline algorithm in above datasets. Owing to 
high-order redundancy being small to have much of an effect on the total usefulness, 
our second-order approximation captures major redundancy and with much lower time 
complexity (compared with baseline). It is worth noting that the time cost of baseline 
is more than one minute (even more than one hour in some datasets) which impedes its 
use in interactive EDA. However, if we do not take redundancy into account in the 
ranking algorithm, i.e., the rank-by-score algorithm, the precision is dropped 
significantly. In summary, our algorithm takes acceptable time and gives a plausible 
ranking result.

==> grammar.tex <==
%{grammar}, needs {obey}

%\newcommand{\heading}[1]{\vspace{3ex}{\noindent#1}\vspace{1.5ex}}
\newcommand{\goesto}{\mbox{$::=$}}
\newcommand{\arbno}[1]{#1\hbox{\rm*}}
\newcommand{\nonterm}[1]{\mbox{$\langle$#1$\rangle$}}

\newenvironment{grammar}{
  \def\:{\goesto{}}
  \def\|{$\vert$}
  \tt \myobeycr%
  \begin{tabbing}%
  \qquad \= $\vert$ \= \qquad \= \kill%
}%
{\unskip\end{tabbing}}

\newenvironment{grammar*}{
  \def\:{\goesto{}}
  \def\|{$\vert$}
  \tt%
  \begin{tabbing}%
  \qquad \= $\vert$ \= \qquad \= \kill%
}%
{\unskip\end{tabbing}}

\newenvironment{roman-grammar}{
  \def\:{\goesto{}}
  \def\|{$\vert$}
  \myobeycr%
  \begin{tabbing}%
  \qquad \= $\vert$ \= \qquad \= \hspace*{5cm} \= \qquad \= \kill%
}%
{\unskip\end{tabbing}}

\newenvironment{roman-grammar*}{
  \def\:{\goesto{}}
  \def\|{$\vert$}
  \begin{tabbing}%
  \qquad \= $\vert$ \= \qquad \= \hspace*{5cm} \= \qquad \= \kill%
}%
{\unskip\end{tabbing}}

\newenvironment{mathGrammar}{
  \def\:{\goesto{}}
  \def\|{\hbox{$\vert$}}
   \begin{displaymath}%
     \tt \obeyspaces%
}%
{\unskip\end{displaymath}}

% Commented grammars

% length before comments start on right
\newlength{\BEFOREGRAMCOMMENTLEN}
\setlength{\BEFOREGRAMCOMMENTLEN}{7cm}

% style of text inside quotations
\newcommand{\GRAMCOMMENTSTYLE}[1]{\texttt{#1}}

\newenvironment{commented-grammar}{%
\begin{grammar}%
\qquad \= $\vert$ \= \qquad \hspace*{\BEFOREGRAMCOMMENTLEN} \= \kill%
}{%
\end{grammar}%
}

\newcommand{\gramcomment}[1]{\textrm{``\GRAMCOMMENTSTYLE{#1}''}}


==> obey.tex <==
%{obey}

% \myobeycr is same as \obeycr, but doesn't do a \@gobblecr.
{\catcode`\^^M=13 \gdef\myobeycr{\catcode`\^^M=13 \def^^M{\\}}%
\gdef\restorecr{\catcode`\^^M=5 }}

% \obeytabs
{\catcode`\^^I=13 \gdef\obeytabs{\catcode`\^^I=13 \def^^I{\hbox{\hskip 4em}}}}

% \obeyspaces
{\obeyspaces\gdef {\hbox{\hskip0.5em}}}

% environment for displayed text, indented, obeys cr, tab, spaces
\newenvironment{obeyDisplay}{%
\samepage%
\begin{list}{}{}\item\obeyspaces\obeytabs\obeycr}{%
\end{list}}

